$ A_\infty $-Deformations and their Derived Categories

Handling curved $ A_\infty $-deformations is challenging and defining their derived categories seems impossible. In this paper, we show how to welcome the curvature and build derived categories despite the apparent difficulties. We explicitly describe their $ A_\infty $-structure by a deformed Kadeishvili theorem. This paper starts with a review of $ A_\infty $-deformations for non-specialists. We explain why $ A_\infty $-deformations require curvature and why curvature supposedly causes problems. We prove that infinitesimally curved $ A_\infty $-deformations are in fact non-problematic and provide the correct definitions for their twisted completion and minimal model. The classical Kadeishvili theorem collapses for curved deformations. We show how to adapt it by iteratively optimizing the curvature and changing the homological splitting infinitesimally. The final $ A_\infty $-structure on the minimal model is constructed in terms of trees.

==> toplevel/notation.tex <==
\section{Notation}
\label{sec:notation}
The following is a list of heavily used notation specific to this paper:

\begin{center}
\begin{longtable}{lll}
Notation & Meaning & Reference \\\hline
\endhead
$ \cat C $ & $ A_∞ $-category & \autoref{def:ainfty-def} \\
$ \cat C_q $ & $ A_∞ $-deformation of $ \cat C $ & \autoref{def:prelim-defo-def} \\
$ μ_q $ & $ μ_{\cat C_q} $, more specifically $ μ_{\Gtl_q Q} $ or $ μ_{\Add \Gtl_q Q} $ & \autoref{def:prelim-defo-def} \\
$ B $ & deformation base & \autoref{def:prelim-defo-base} \\
$ \mathfrak{m} $ & maximal ideal of $ B $ & \autoref{def:prelim-defo-base} \\
$ B \htensor V $ & completed tensor product with vector space $ V $ & \autoref{def:prelim-htensor-def} \\
$ \mathfrak{m} V $ & shorthand for $ \mathfrak{m} \htensor V ⊂ B \htensor V $ & \autoref{def:prelim-htensor-def} \\
$ \Tw\cat C_q $ & twisted completion of $ \cat C_q $ & \autoref{def:curved-twisted} \\
$ \Tw'\cat C_q $ & liberal twisted completion of $ \cat C_q $ & \autoref{th:twisted-deforming-delta} \\
$ \H\cat C_q $ & minimal model of $ \cat C_q $ & \autoref{th:kadeishvili-existence-th} \\
$ \mathcal{T} $ & set of Kadeishvili tree shapes & \autoref{def:kadeishvili-classical-treeshape} \\
$ N_T $ & number of internal nodes of a tree & \autoref{def:kadeishvili-classical-treeshape} \\
$ φ $ & bijection $ H_q → B \htensor H $ & \autoref{def:kadeishvili-deformed-counterpart} \\
$ F: \cat C → \cat D $ & $ A_∞ $-functor & \autoref{def:curved-functors-ainftyfunctor} \\
$ F_q: \cat C_q → \cat D_q $ & functor of deformed $ A_∞ $-categories & \autoref{def:curved-functors-def} \\
$ \MC(L, B) $ & Maurer-Cartan elements of DGLA/$ L_∞ $-algebra & \autoref{def:curved-hochschild-MC} \\
$ \MCb(L, B) $ & $ \MC(L, B) $ modulo gauge equivalence/homotopy & \autoref{def:curved-gauge-def} \\
$ \HC(\cat C) $ & Hochschild DGLA of $ \cat C $ & \autoref{def:curved-hochschild-HC} \\
$ (S, M) $ & punctured surface & \autoref{def:prelim-punctured-def} \\
$ \cA $ & arc system & \autoref{def:prelim-arcsys-def} \\
$ a $ & arc in $ \cA $ & \autoref{def:prelim-arcsys-def} \\
$ h(a), t(a) $ & puncture at head/tail of arc $ a $ & \autoref{def:prelim-arcsys-def} \\
$ α $ & angle in $ \cA $ & \autoref{def:prelim-gtl-gtl-def} \\
$ h(α), t(α) $ & arc at head/tail of angle $ α $ & \autoref{def:prelim-arcsys-def} \\
$ Q $ & dimer, typically geometrically consistent & \autoref{def:prelim-gtl-dimers-def} \\
$ Q_M $ & standard sphere dimer & \autoref{sec:sphere-zigzagcat} \\
$ \id_a $ & arc identity & \autoref{sec:prelim-gtl-gtl} \\
$ L $ & zigzag path & \autoref{def:prelim-gtl-zigzag-def} \\
$ \ZigzagCat $ & zigzag category & \autoref{def:splitting-zigzagcat-def} \\
$ \DefZigzagCat $ & deformed zigzag category & \autoref{def:deformed-zigzagcat-def} \\
$ a_0 $ & identity location on zigzag path & \autoref{conv:alpha0-direction} \\
$ α_0 $ & co-identity location on zigzag path & \autoref{conv:alpha0-direction} \\
$ P_k $ & standard $ k $-gon & \autoref{sec:prelim-gtl-infty} \\
$ ε $ & elementary morphism $ ε: L_1 → L_2 $ & \autoref{sec:prelim-terminology} \\
$ T $ & Kadeishvili tree shape & \autoref{sec:kadeishvili-classical} \\
$ T $ & tail of a morphism $ ε: L_1 → L_2 $ & \autoref{def:deformed-tails-tail} \\
$ \PiTr $ & class of result components of π-trees & \autoref{def:subdisk-shapeless-def} \\
$ \SLd $ & class of shapeless disks & \autoref{def:subdisk-shapeless-def} \\
$ \CRr $ & class of CR result components & \autoref{def:subdisk-types-rescomp} \\
$ \IDr $ & class of ID result components & \autoref{def:subdisk-types-rescomp} \\
$ \DSr $ & class of DS result components & \autoref{def:subdisk-types-rescomp} \\
$ \DWr $ & class of DW result components & \autoref{def:subdisk-types-rescomp} \\
$ \CRd $ & class of CR disks & \autoref{def:subdisk-types-CRdisk} \\
$ \IDd $ & class of ID disks & \autoref{def:subdisk-types-IDdisk} \\
$ \DSd $ & class of DS disks & \autoref{def:subdisk-types-DSdisk} \\
$ \DWd $ & class of DW disks & \autoref{def:subdisk-types-DWdisk} \\
$ \Subdisk $ & subdisk mapping $ \Subdisk: \PiTr → \SLd $ & \autoref{th:subdisk-subdisk-Dconstruction} \\
$ \disktarget(D) $ & target/output morphism of disk $ D $ & \autoref{def:subdisk-shapeless-def} \\
$ \Abouzaid(D) $ & Abouzaid sign of disk $ D $ & \autoref{def:subdisk-minmodel-Abouzaid} \\
$ \punctures(D) $ & product of punctures covered by $ D $ & \autoref{def:subdisk-minmodel-Abouzaid}
\end{longtable}
\end{center}

